Towards a General Time Series Anomaly Detector with Adaptive Bottlenecks and Dual Adversarial Decoders

Time series anomaly detection plays a vital role in a wide range of applications. Existing methods require training one specific model for each dataset, which exhibits limited generalization capability across different target datasets, hindering anomaly detection performance in various scenarios with scarce training data. Aiming at this problem, we propose constructing a general time series anomaly detection model, which is pre-trained on extensive multi-domain datasets and can subsequently apply to a multitude of downstream scenarios. The significant divergence of time series data across different domains presents two primary challenges in building such a general model: (1) meeting the diverse requirements of appropriate information bottlenecks tailored to different datasets in one unified model, and (2) enabling distinguishment between multiple normal and abnormal patterns, both are crucial for effective anomaly detection in various target scenarios. To tackle these two challenges, we propose a General time series anomaly Detector with Adaptive Bottlenecks and Dual Adversarial Decoders (DADA), which enables flexible selection of bottlenecks based on different data and explicitly enhances clear differentiation between normal and abnormal series. We conduct extensive experiments on nine target datasets from different domains. After pre-training on multi-domain data, DADA, serving as a zero-shot anomaly detector for these datasets, still achieves competitive or even superior results compared to those models tailored to each specific dataset. The code is made available at https://github.com/decisionintelligence/DADA.

==> Sections/reproducibility.tex <==
\section*{Reproducibility Statement}

In this work, we have made every effort to ensure reproducibility.

In our supplementary materials, we include code and evaluation datasets that are complete, well-documented, and easily accessible. Within the code files, we provide script files to facilitate running and reproducing our experimental results. 
In Methodology~\ref{Methodology}, from input to output, we provide a detailed description of our method, including model structure, model training, and anomaly criterion. 
In Appendix.~\ref{app:IMPLEMENTATION DETAILS}, we summarize all the default hyper-parameters, including patch size, learning rate, etc. 
In Appendix.\ref{app:DATASETS}, we describe all the datasets used in the pre-training and testing of our method. The code is made available at \url{https://anonymous.4open.science/r/DADA-FDBF}.


==> table/bn_moe.tex <==
\begin{tabular}{c|c|c|c|c|c}
\hline \hline
\textbf{Models} & {\textbf{SMD}} & {\textbf{SMAP}}    & {\textbf{MSL}} & {\textbf{SWaT}}  & {\textbf{PSM}}\\ \hline
\textbf{fix}
& 76.73 & 68.73 & 68.01 & 71.12 \\
\textbf{W/O ABN} 
& 79.50 & 74.55 & 69.29 & 74.45\\
\textbf{W/O Adversarial} 
& 61.59 & 63.83 & 64.28 & 63.23\\
\textbf{W/O Dual Decoder} 
& 83.03 & 74.47 & 72.62 & 76.70
\\ \hline
\textbf{DADA}
& \textbf{84.57} & \textbf{78.48} & \textbf{75.42} & \textbf{79.49}\\ \hline 
\hline
\end{tabular}

==> table/multi-metrics.tex <==
\begin{tabular}{c|ccccc|ccccc}
\hline \hline
\textbf{Dataset} & 
\multicolumn{5}{c|}{\textbf{NeurIPS\_TS}} & 
\multicolumn{5}{c}{\textbf{Daphnet}} \\ \hline
\textbf{Method} & 
\textbf{Acc} & \textbf{F1} & \textbf{A\_R} & \textbf{R\_A\_R} & \textbf{V\_ROC} & 
\textbf{Acc} & \textbf{F1} & \textbf{A\_R} & \textbf{R\_A\_R} & \textbf{V\_ROC} \\ \hline
A.T.
& 81.03 & 58.79 & 40.00 & 59.89 & 58.29 
& \underline{90.18} & 70.03 & 38.61 & 37.41 & 37.27 
\\  
DCdetector
& 89.87 & 53.90 & 47.46 & 69.05 & 66.41 
& \textbf{90.35} & 70.14 & 41.86 & 43.63 & 43.54 
\\
D3R 
& 80.34 & 62.46 & 63.40 & 79.83 & 78.98 
& 74.29 & 56.03 & 32.93 & 38.14 & 41.66
\\  
ModernTCN 
& 89.78 & 63.14 & \underline{77.37} & \textbf{85.48} & \textbf{85.12}
& 87.19 & 75.08 & 70.93 & 74.85 & 74.57 
\\
GPT4TS 
& \underline{89.94} & \underline{65.56} & 76.66 & 83.92 & 83.89 
& 86.73 & \underline{76.07} & \textbf{72.99} & \underline{77.13} & \underline{76.92} 
\\ \hline
DADA (\textcolor{red}{zero shot}) 
& \textbf{90.04} & \textbf{68.23} & \textbf{77.81} & \underline{83.98} & \underline{83.91}
& 87.10 & \textbf{76.10} & \underline{72.86} & \textbf{77.29} & \textbf{76.93}
\\ \hline
\hline
\end{tabular}
